Impacts of Primordial Black Holes in the Early Universe

The work presented in this thesis draws back the curtain on the physics of the primordial universe by leveraging Primordial Black Holes (PBHs) as cosmological probes. The violent deaths of ultralight PBHs are shown to severely inhibit leptogenesis, alter the sphaleron freeze-out temperature and provide an opportunity to rule out models of leptogenesis which would otherwise evade direct detection experiments for effective eternity. Turning to the extreme temperature gradients of hot spots, the evolution and formation of hot spots was considered in an expanding background for the first time, and a formalism treating the propagation of Hawking radiation was introduced. Upon addressing the previously unexplored effects of hot spots on Hawking radiation, it was discovered that hot spots can support successful leptogenesis after sphaleron freeze-out, and efficiently absorb radiated Dark Matter. These examples hint at an intricate, rich tapestry of physics in hot spots.

==> Chapter_1/Baryogenesis/EW.tex <==
Show that each of Sakharov's conditions is satisfied in the SM. 
\subsubsection{sphalerons in the SM}
Show that EW baryogenesis is excluded by the measurement of the Higgs mass

==> Chapter_1/Baryogenesis/Explanations.tex <==

Feasibility of initial conditions argument. Argument for dynamic generation. Sakharov's conditions

==> Chapter_1/Baryogenesis/GUT.tex <==

General formulation of GUT scale baryogenesis in terms of generic $X$ particle. Proton decay, possible candidates.

==> Chapter_1/Cosmology/Early_Universe.tex <==

\subsubsection{Einstein's Field Equations}
Derive Friedmann Eqn from the Field Equations. 
\subsubsection*{Radiation}
\subsubsection*{Matter}
\subsubsection*{Dark Energy/Vacuum} 

==> Chapter_1/Cosmology/History.tex <==
\subsubsection{Mixed constituent model}
Standard case, discuss CMB evidence of relative abundances today


==> Chapter_1/Cosmology/Inflation.tex <==
Motivation for inflation. Canonical single-field formulation. Density perturbation


\subsubsection{The scalar power spectrum}
How models affect predictions for power spectra, GWs
\subsubsection{Reheating}
Parametric resonance and population of the SM fields. Introduce necessary computational tools to later discuss vanishing initial conditions case

==> Chapter_1/Cosmology/LCDM.tex <==
$\Lambda CDM$ overview, cosmological principle and FRLW metric. 
\subsubsection{Predictions of $\Lambda CDM$}
The CMB power spectrum, N-body simulations








==> Chapter_1/Early_Universe/Phase_Transitions.tex <==
\begin{itemize}
    \item EWPT temperature
\end{itemize}

==> Chapter_1/Leptogenesis/Flavour.tex <==
\begin{itemize}
    \item leptons distinguished by Yukawas
    \item effects on thermal mass
    \item Temperature range of importance
    \item  impact of flavour effects
\end{itemize}




The definition of the parameter $\epsilon_{\iflav \iflav}$ given in \equaref{Leptogenesis/CP/epsilon} describes the relative CP asymmetry in the decay of $N_i$ into lepton flavour $\iflav$. At the Lagrangian level the SM leptons are distinguished by their Yukawa couplings $h_\iflav$, which mediate elastic scattering interactions in the early universe. These processes produce neither lepton asymmetry nor RHNs and are generally spectator processes. However as shown in \secref{Leptogenesis/Thermal}, when fast compared to the Hubble rate they ought to generate thermal masses for the SM leptons. The charged lepton Yukawas vary greatly in size and so one would expect similarly disparate thermal masses. Estimating the charged lepton Yukawa interaction rate as 
\begin{equation}
    \Gamma_\iflav \approx 5\times 10^{-3} h_\iflav^2 T
\end{equation}
it turns out that for $T \gtrsim 10^{12}$\,GeV none of the charged lepton Yukawa interactions are fast compared to the Hubble rate \cite{Davidson:2008bu}. At extremely high temperatures therefore, the total BAU could be calculating by summing \equaref{Leptogenesis/CP/epsilon} over the flavour index $\epsilon = \sum_\iflav \epsilon_{\iflav \iflav}$, leptogenesis is blind to lepton flavour and the total asymmetry evolves as if in a single flavour.

==> Chapter_2/LeptoPapers.tex <==




%==================================================
\section{High-scale leptogenesis model}\label{sec:HSL}
%==================================================

In this section, we outline the high-scale, thermal leptogenesis mechanism used throughout our analysis. Thermal leptogenesis is based on a minimal extension of the Standard Model (SM) comprising at least two singlet Majorana neutrinos which couple to the SM lepton and Higgs doublets. An attractive feature of this minimal model is the simultaneous explanation of the neutrino masses experimentally measured~\cite{Capozzi:2021fjo, Esteban:2020cvm, deSalas:2020pgw} and the baryon asymmetry of the Universe.




\subsection*{CP asymmetry}
 
With this simplification, the CP asymmetry parameter $\epsilon$ can be expressed in terms of only four unknown parameters $\{x,y, m_h, M_1\}$\,\cite{Bernal:2022pue}
\begin{equation}
    |\epsilon| = \frac{3M_1}{16\pi v_{EW}^2}\frac{|\Delta m^2_{\rm atm}|}{m_h + m_l}\frac{|\sin(2x)\sinh(2y)|}{\cosh(2y) - f\cos(2x)}\,,
\end{equation}
where $f \equiv (m_h - m_l)/(m_h + m_l)$ with $m_h = m_3$ and $m_l = m_1 \approx m_2$. While $\epsilon$ controls the amount of CP violation associated with the decay of $N_1$ particles, their thermal production violates CP with the same magnitude and opposite sign. Therefore when there is a vanishing initial abundance of $N_1$, an initial ``anti-asymmetry" is produced in the leptons. After reaching the thermal distribution, the population of $N_1$ will then decay when the temperature of the Universe is $T=M_1$, as long as the decay rate at that time is faster compared to the Hubble parameter. Such a condition is equivalent to~\cite{Strumia:2006qk,Davidson:2008bu, Buchmuller:2004nz}
\begin{equation}\label{K}
    K\equiv \frac{\tilde{m}_1}{m^*} > 1,
\end{equation}
where
\begin{equation}\label{meff}
    m^* = \frac{8\pi v_{EW}^2}{M_1^2} H\left(T=M_1\right)\,,
\end{equation}
and
\begin{equation}
    \tilde{m}_i = \sum_\alpha \frac{|Y_{\alpha\,i}|^2v_{EW}^2}{M_i}\,,
\end{equation}
representing the expansion rate at $T=M_1$ and the decay rate, respectively. When the right-handed neutrinos decay out of equilibrium, the resulting asymmetry would exactly cancel against the initial anti-asymmetry, if it were not for the so-called ``washout" processes which are crucial to leptogenesis.

Washout processes include the inverse decay modes of $N_1$, {\it i.e.} $\ell \phi^\dagger \to N_1$ and $\bar{\ell} \phi \to N_1 $, which are Boltzmann suppressed at low temperatures and do not contribute to the asymmetry, but are important at $T\sim M_1$ since they deplete the initial anti-asymmetry. Also important are $2\leftrightarrow2$ scattering processes like $\ell \phi^\dagger \to \bar{\ell} \phi $ mediated by $N_1$ exchange that do not suffer the same Boltzmann suppression since the intermediate state $N_1$ can go off-shell. For $K > 1$, the $N_1$ population decays when these processes are effective, so a non-zero lepton asymmetry survives since they wash out the initial anti-asymmetry, precluding any cancellation. For this reason, the condition $K > 1$ defines the ``strong-washout" regime. In the opposite regime $K < 1$, the decays are slow compared to the Hubble rate at $T = M_1$ and the $N_1$ population decays at a later time when the washout processes are weak, leading to a cancellation with the initial anti-asymmetry. In the weak-washout regime it is generally required to introduce a further mechanism to produce an initial population of $N_1$ to avoid this~\cite{Davidson:2008bu}. It is also interesting to note that the neutrino masses suggested by experiments favour the strong-washout regime since the weak-washout regime only appears for $m_h$ very close to $\sqrt{\Delta m^2_{\rm atm}}$. In our analysis, we always work in the strong-washout regime, so we require $|y| > 0.14$. This also means that any contribution to the asymmetry from $N_{2,3}$ is suppressed due to being washed out at $T\ll M_1$. 
\begin{figure*}[t!]
    \centering
    \includegraphics[width = 0.3 \textwidth]{Figures/LeptoPaper1/y_vs_x_0.05.pdf}
    \includegraphics[width = 0.3 \textwidth]{Figures/LeptoPaper1/y_vs_x_0.1.pdf}
    \includegraphics[width = 0.3 \textwidth]{Figures/LeptoPaper1/y_vs_x_0.2.pdf}
    \caption{\label{xy}The final baryon asymmetry $\YB$ as a function of $x, \,y$ for $m_h = \sqrt{m_{\rm atm}^2} \approx 0.05$~eV (left panel), $m_h = 0.1$~eV (middle panel) and $m_h = 0.2$~eV (right panel), with $M_1 = 2.0 \times 10^{13}~{\rm GeV}$. The contours are for constant $\log_{10} \YB$ while the symbol $\odot$ indicates the point $(x,y)$ which maximises $\YB$ for the fixed values of $m_h$.}
\end{figure*}

\subsection*{Boltzmann equations}
To calculate the baryon asymmetry of the Universe, we solve numerically the Boltzmann equations describing the number density of $N_1$, and the $B-L$ asymmetry where $B$ and $L$ are the total baryon and lepton numbers of the Universe, respectively. It is convenient to track the evolution of the $B-L$ asymmetry since it is conserved by the sphaleron processes which partially convert the lepton asymmetry into a baryonic one.

In our analysis, we assume a vanishing initial abundance of $N_1$ and $B-L$ and we account for the following types of processes:
\begin{itemize}
    \item $1\to 2$ decays of $N_1$, $N_1 \to \ell \phi^\dagger$ and its CP conjugate process $N_1 \to \bar{\ell} \phi$. The total rates are proportional to the number density of $N_1$ and the thermally averaged decay width. Decays deplete the population of $N_1$ and contribute a source term to the $B-L$ asymmetry.
    %
    \item $2 \to 1$ inverse decay modes like $\ell \phi^\dagger \to N_1$. The inverse decay rate is related to the decay rate by $\Gamma^{ID}_{N_1} = \Gamma_{N_1}n_{N_1}^{\rm eq}/n^{\rm eq}_{\ell}$ where $n_{N_1}^{\rm eq},n^{\rm eq}_{\ell}$ are the equilibrium number densities of $N_1$ and the leptons. These processes produce the $N_1$ population but only wash out the asymmetry.
    %
    \item $2 \leftrightarrow 2$ scatterings mediated by $N_1$ exchange like $\ell \phi^\dagger \to \bar{\ell} \phi$, for which $\Delta L = 2$. These processes contribute to the washout and do not change the number density of $N_1$. Care should be taken when combining $2\leftrightarrow 2$ scatterings in the s-channel and the inverse decay rates to avoid double counting. A subtracted form of the amplitude should be used which only accounts for off-shell $N_1$ exchange, so these processes are not Boltzmann suppressed at low energies.
\end{itemize}
In principle one should also account for $2\leftrightarrow 2$ scatterings involving the gauge bosons and top quarks, but since these are order $(Y^2 Y_t^2)$ or higher in the couplings, where $Y_t$ is the top quark Yukawa coupling, we neglect them here. The effects of 3-body decay processes are also numerically small, $\sim 6\%$, and can be ignored~\cite{Nardi:2007jp}.

In standard $\Lambda$CDM cosmology, the resulting Boltzmann equations for the comoving number density of $N_1$ and $B$-$L$ are
\begin{eqnarray}
\frac{{\rm d}\NNo}{{\rm d}\alpha} &=&\ln(10)  \frac{\GN}{H}(\NNeqo-\NNo)\,, \label{eq:Nth} \\
\frac{{\rm d} \NBL} {{\rm d}\alpha} &=&   \left.\frac{\ln (10)}{H}\right[ \epsilon(\NNo-\NNeqo)\GN + \\ \nonumber
&&\qquad \left. + \left(\frac{1}{2} \frac{\NNeqo}{\Nleq}\GN + \gamma \frac{a^3}{\Nleq}\right)  \NBL\right]\,,\label{AsymBoltzmann}
\end{eqnarray}
where $\NNo = n_{N_1}a^3$, $\NBL = n_{\rm B-L}a^3$, $H = \Dot{a}/a$ is the Hubble rate and 
\begin{equation}
\alpha \equiv \log_{10}(a) \,,
\end{equation}
with $a$ being the scale factor. 

In Eq.~\eqref{AsymBoltzmann}, $\gamma$ quantifies the contribution to the washout associated with the $\Delta L = 2$ scattering processes. In Ref.\,\cite{Bernal:2022pue} it is shown that 
\begin{equation}
    \gamma = \frac{3T^6}{4\pi^5 v_{EW}^4} \mathrm{Tr}[m_\nu^\dagger m_\nu]\,.
\end{equation}
Since the right-handed neutrino mass is much larger than the temperature of the electroweak phase transition $T_{\rm EWPT} \approx 160~{\rm GeV}$~\cite{DOnofrio:2015gop}, the lepton asymmetry stops evolving when the washout processes go out of equilibrium at temperatures far above the sphaleron freeze-out. The baryon asymmetry is then frozen-in when the sphaleron processes go out of equilibrium at $T = T^{\rm sph}$~\cite{DOnofrio:2014rug}, giving a yield of baryons today defined by \equaref{YB}


\subsection*{The parameter space of high-scale leptogenesis}
All of the relevant quantities in Eq.s~\eqref{eq:Nth} and~\eqref{AsymBoltzmann}, and in particular today’s baryon asymmetry, can be now calculated in the four-dimensional parameter space $\{x,y, m_h, M_1\}$. We consider the following parameter ranges:
\begin{eqnarray}
0<x<\pi & \quad{\rm and}\quad & 0.14<y<\pi \label{range1}\\
0.05 < \frac{m_h}{{\rm eV}} < 0.8 & \quad{\rm and}\quad & 10^{10}< \frac{M_1}{{\rm GeV}} < 10^{16}\nonumber
\end{eqnarray}
The bound $y>0.14$ ensures the strong-washout regime in all the parameter space considered. The lower bound for the heaviest active neutrino mass $m_h$ comes from the neutrino oscillation data requiring $m_h > \sqrt{m_{\rm atm}^2}\approx 0.05~{\rm eV}$~\cite{Capozzi:2021fjo, Esteban:2020cvm, deSalas:2020pgw}, while the upper bound is set by the KATRIN experiment~\cite{KATRIN:2021uub}.

In Fig.~\ref{xy} we show the dependence of $\YB$ on the angles $x, \,y$ taking $M_1=2.0 \times 10^{13}~{\rm GeV}$, for three different active neutrino masses: $m_h = \sqrt{m_{\rm atm}^2} \approx 0.05$~eV (left panel), $m_h = 0.1$~eV (middle panel) and $m_h = 0.2$~eV (right panel). In the plots, the contours represent different values of $\log_{10} \YB$. Moreover, the symbol $\odot$ indicates the point $(x,y)$ which maximises $\YB$. For $m_h \gg \sqrt{m_{\rm atm}^2}$, the asymmetry $|\YB|$ is always maximised for $y = 0.44$ and $x = \pi/4$~\cite{Bernal:2022pue} (middle and right panels), while for smaller $m_h$ (left panel) the dependence on the angles $x,y$ is non-trivial requiring us to perform a detailed numerical scan. Between these two regimes, the point maximising $\YB$ is continuously translated from the position on the left panel to that on the right panel. As it will be detailed in the next section, the evaporation of primordial black holes leads to an entropy injection which dilutes the baryon asymmetry produced by leptogenesis. For this reason, we scan the parameter space to find the points which maximise the baryon asymmetry $\YB$. In particular, we choose to always fix the angles $x,y$ to maximise the final baryon asymmetry defining the quantity
\begin{equation}\label{YBm}
    \YBm(m_h,M_1)=\max_{x,y} \YB (x,y,m_h,M_1)\,.
\end{equation}
\begin{figure*}[t!]
    \begin{minipage}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]
    {Figures/LeptoPaper1/mN_vs_mh.pdf}
    \end{minipage}%
    \hspace{0.05\linewidth}
    \begin{minipage}[b]{0.25\linewidth}
    \centering
    \begin{tabular}[b]{c|c|c|c}
        Bench. pt & $m_h~[{\rm eV}]$ & $M_1~[{\rm GeV}]$ & $\YBm$ \\ \hline
         {\bf 1} & $0.05$ & $1.5 \times 10^{14}$ & $1.5 \times 10^{-6} $ \\ \hline
         {\bf 2} & $0.07$ & $1.0 \times 10^{14}$ & $3.6 \times 10^{-9} $ \\ \hline
         {\bf 3} & $0.10$ & $4.0 \times 10^{13}$ & $5.5 \times 10^{-10}$ \\ \hline
         {\bf 4} & $0.14$ & $2.0 \times 10^{13}$ & $1.2 \times 10^{-10}$ \\ 
    \end{tabular}
    \vspace{80pt}
    \end{minipage}
    \hspace{0.05\linewidth}
    \caption{\label{fig:Ybm}The quantity $\YBm$ defined in Eq.~\eqref{YBm} as a function of $m_h$ and $M_1$. The dashed contour marks the observed baryon asymmetry of the Universe, while the dotted ones represent larger values as reported in the labels. The solid line shows the parameters that maximise the baryon asymmetry, with points from 1 to 4 highlighting the benchmark cases reported in the table on the right. The grey bands are excluded by experimental limits from oscillation data~\cite{Capozzi:2021fjo, Esteban:2020cvm, deSalas:2020pgw} (left) and KATRIN searches~\cite{KATRIN:2021uub} (right).}
\end{figure*}

In Fig.~\ref{fig:Ybm}, we report the maximum baryon asymmetry $\YBm$ in colour, as a function of the heaviest left and
lightest right handed neutrino mass scales. The dashed line represents the parameters for which $\YBm$ matches the observed value reported in Eq.~\eqref{YBexp}. It also delimits from the right the region in the parameter space where the high-scale thermal leptogenesis can correctly account for the baryon asymmetry of the Universe. Indeed, in that region the observed value $\YB^{\rm obs}$ can be achieved by simply tuning the angles $x,y$. In the plot, we also show different increasing values for the ratio $\YBm/\YB^{\rm obs}$ with dotted lines. Moreover, the solid line represents the relation between $m_h$ and $M_1$ that maximises the baryon asymmetry $\YB$. The numbered points highlight benchmark cases for different active neutrino mass $m_h$ that will be used as reference in later plots. For each value of $M_1$, the final baryon asymmetry increases for decreasing $m_h$. We find that the the maximal allowed value for the baryon asymmetry in the high-scale thermal leptogenesis scenario is
\begin{equation}\label{benchmark}
\YB^{\rm max} = 1.5\times 10^{-6}
\end{equation}
achieved for $x=1$, $y = 0.14$, $m_h = 0.05~{\rm eV}$ and $M_1 = 1.5 \times 10^{14}\,{\rm GeV}$.
For this choice of parameters, an entropy production of about four orders of magnitude at later times (e.g. from PBHs' evaporation) would be required to obtain the observed baryon asymmetry of the Universe (see Eq.~\eqref{YBexp}). A larger amount of entropy production would be in tension with the high-scale thermal leptogenesis giving $\YB < \YB^{\rm obs}$.




%==================================================
\section{Results}\label{sec:res}
%==================================================
\begin{figure*}[t!]
    \centering
        \includegraphics[width = 0.49\textwidth]{Figures/LeptoPaper1/benchmark_11.pdf}
        \includegraphics[width = 0.49\textwidth]{Figures/LeptoPaper1/benchmark_12.pdf}
       \caption{\label{fig:benchmark} The yield $Y_{\rm B-L}$ as a function of $z=M_1/T$ (top panels) with and without the presence of PBHs taking $\MPBH = 10^6~{\rm g}$ (left plot) and $\MPBH = 10^8~{\rm g}$ (right plot). The PBH initial abundance is fixed in order to obtain the observed baryon asymmetry (solid grey horizontal line) after PBH evaporation. The neutrino parameters are fixed according to the benchmark case 1 in Fig.~\ref{fig:Ybm}. The middle and bottom panels show the evolution of energy densities and the entropy ratio $\Sr$.}
\end{figure*}
\begin{figure*}[t!]
    \centering
        \includegraphics[width = 0.49\textwidth]{Figures/LeptoPaper1/benchmark_41.pdf}
        \includegraphics[width = 0.49\textwidth]{Figures/LeptoPaper1/benchmark_42.pdf}
       \caption{\label{fig:benchmark2} Same as in Fig.~\ref{fig:benchmark} but fixing the neutrino parameters according to the benchmark case 4 reported in Fig.~\ref{fig:Ybm}.}
\end{figure*}

Our model is described by six free parameters: four are needed to describe the leptogenesis mechanism $\{x,\,y,\, m_h,\,  M_1\}$, taken in the range in Eq.~\eqref{range1}, and two parameters that describe PBH physics $\{\MPBH,\, \beta^\prime\}$ in the range 
\begin{equation}
    10^6 < \MPBH/ {\rm g} < 10^9 \qquad {\rm and} \qquad 10^{-15}< \beta^\prime <0.1
    \label{range2}
\end{equation}
As already discussed, we perform a scan on the free parameters to identify the maximum $\YB$ attainable for fixed combinations of $m_h$ and $M_1$ (see Eq.~\eqref{YBm}). For each choice of point in our parameter space, we solve the two coupled equations~\eqref{eq:Nth} and~\eqref{AsymBoltzmann}, then by means of Eq.~\eqref{YB} we obtain $\YB$ today. The results are reported in Fig.s~\ref{xy} and~\ref{fig:Ybm}. Then, for each choice of $\MPBH$ and $\beta^\prime$, by solving Eq.s~\eqref{eq:FE_PBH} and~\eqref{eq:entropy}, we can derive the entropy injection from PBH complete evaporation and quantify the dilution of baryon asymmetry.

In Fig.s~\ref{fig:benchmark} and~\ref{fig:benchmark2}, we show how the presence of light PBHs alters the evolution of the $B$-$L$ yield (top panel) as a function of the auxiliary variable $z = M_1/T$. In the former figure, we fix the neutrino parameters according to the benchmark point 1 in Fig.~\ref{fig:Ybm}, while in the latter they correspond to the benchmark point 4. In the left (right) plots, the PBH mass is taken be to $10^6~{\rm g}$ ($10^8~{\rm g}$), with their initial abundance $\beta^\prime$ fixed to achieve the observed baryon asymmetry after evaporation. In the top panels of the plots, the dashed lines correspond to the standard evolution without PBHs for which the final asymmetry is higher than the observed one represented by the solid horizontal grey lines. We also report the evolution of the energy densities of radiation and PBHs (middle panels) and the ratio $\Sr$ (bottom panels). The left (right) plot refers to the benchmark point 1 (4) reported in the table in Fig.~\ref{fig:Ybm} with an initial PBH abundance of $\beta^\prime = 10^{-9}$ ($\beta^\prime = 3 \times 10^{-14}$). In Fig.~\ref{fig:benchmark} (benchmark point 1), PBHs rule a matter-dominated phase until they evaporate leading to a large entropy injection. In Fig.~\ref{fig:benchmark2} (benchmark point 4), even though PBHs never dominate the energy content of the Universe, their evaporation dilutes the final baryon asymmetry to match the observed value. In these benchmark cases, as well as in the whole PBH mass range considered (see Eq.~\eqref{range2}), the PBH evaporation occurs after the sphaleron processes freeze-out at $z = z_{\rm sph}$ (vertical dotted lines) and before the beginning of BBN at $T \simeq 1~{\rm MeV}$. Therefore, PBHs mainly modify the cosmological evolution only after the $B$-$L$ asymmetry has already been generated via leptogenesis. We note that the energy density of PBHs linearly depends on their initial abundance $\beta^\prime$. This implies that values for $\beta^\prime$ larger than the ones adopted in such benchmark cases would lead to $\YBm < \YB^{\rm obs}$ and consequently would be in tension with the minimal high-scale leptogenesis scenario.

\begin{figure}[t!]
    \centering
        \includegraphics[width =\linewidth]{Figures/LeptoPaper1/Constraints.pdf}
        \caption{\label{fig:constraints}Mutual exclusion limits between PBHs and the minimal high-scale leptogenesis in the $\MPBH$-$\beta^\prime$ plane. The different colors correspond to the upper bounds obtained assuming different masses $m_h$ for the heaviest active neutrino, while the other neutrino parameters are fixed to maximise the baryon asymmetry. The numbered dashed lines refer to the benchmark cases reported in Fig.~\ref{fig:Ybm}. The hatched region is excluded according to the constraints on the GW energy density from BBN observations~\cite{Domenech:2020ssp}. The shaded grey region highlights PBHs whose evaporation occurs during BBN.}
\end{figure}

The main results of our analysis are displayed in Fig.~\ref{fig:constraints} where we report the mutual exclusion limits between PBHs and high-scale leptogenesis projected in the PBH parameter space. In particular, for each active neutrino mass $m_h$ we derive an upper bound in the PBH parameter space further fixing the right-handed neutrino mass $M_1$ to maximise the baryon asymmetry. In the leptogenesis parameter space, this corresponds to considering the values along the solid black line in Fig.~\ref{fig:Ybm}. Indeed, the four numbered dashed lines refers to the four benchmark cases in Fig.~\ref{fig:Ybm}. The maximum allowed asymmetry in the minimal high-scale leptogenesis decreases as $m_h$ increases, thus placing stronger constraints on $\beta^\prime$. The strongest upper bound on $\beta^\prime$ (darkest violet line) corresponds to the highest possible value for $m_h$ so that the observed baryon asymmetry is achieved. Conversely, the conservative constraint (darkest red line) is set for the lowest possible value for $m_h\approx 0.05~{\rm eV}$ according to neutrino oscillation data. We find that such a conservative bound is stronger than the one imposed by the limit on the energy density of gravitation waves (GWs) at the time of BBN~\cite{Domenech:2020ssp, Papanikolaou:2020qtd} (hatched area in the plot). In the figure, we also highlight the shaded grey area where PBHs would evaporate and dilute the baryon asymmetry during BBN.


%==================================================
\section{Conclusions}\label{sec:concl}
%==================================================

We investigate the impact of the non-standard cosmology driven by the presence and the evaporation of light primordial black holes on the production of the baryon asymmetry of the Universe through high-scale leptogenesis. Crucially, the evaporation of PBHs is associated with (a sudden) injection of entropy and reheating of the Universe. When this occurs after the sphaleron freeze-out, the baryon asymmetry is diluted. In this framework, we firstly explore the four-dimensional parameter space of high-scale leptogenesis in its minimal version demonstrating the existence of a finite, maximum achievable asymmetry $\YB^{\rm max}$. We then point out that, if the entropy injection from primordial black holes' evaporation is large enough, even $\YB^{\rm max}$ does not reproduce the observed asymmetry of the Universe. This effectively rules out high-scale leptogenesis as the baryogenesis mechanism. In this fashion, we derive mutual exclusion limits in the PBH and leptogenesis parameter spaces, delineating the regions which are incompatible. For an entropy increase greater than around four orders of magnitude, the minimal model for high-scale leptogenesis is insufficient to account for the baryon asymmetry of the Universe. This corresponds to a PBH population with masses from $10^6$ to $10^9$ grams with an initial abundance $\beta^\prime > 10^{-9}$. Interestingly, we point out the existence of a relation between the heaviest active neutrino mass $m_h$ and the conservative bound in the PBH parameter space which results to be stronger than existing constraints.




















\section*{Low Scale Leptogenesis}



%================================
\section{Sub-TeV resonant leptogenesis \label{sec:leptogenesis}}
%================================

In this section we overview the mechanism of sub-TeV resonant leptogenesis describing the main parameters (connected to the seesaw mechanism for the neutrino mass and mixing generations) and the relevant Boltzmann equations. Moreover, we discuss the parameter space achieving the correct baryon asymmetry of the Universe.

\subsection*{Type-I seesaw}

One of the simplest mechanisms to generate neutrino masses is the type-I seesaw, in which the SM is minimally extended by $n$ Majorana singlet fermions, the Right-Handed Neutrinos (RHNs), $N_i$ with $i=1,...,n$, which mix with the SM leptons through their Yukawa couplings to the Higgs. The simplest case is $n=2$ predicting the lightest active neutrino to be massless. However, ${\rm SO}(10)$ models predict $n=3$, and in general having the same number of left and right handed neutrino fields is a quite common assumption. Here, we assume $n=3$ and consider two nearly degenerate RHNs ($M\sim M_1 \sim M_2$) with a tiny mass splitting $\Delta M = M_2 - M_1 \ll M_{1,2}$ and a third effectively decoupled RHN ($M_3 \gg M$). 

 

 Moreover, we assume the two neutrino Majorana phases to be zero and  we consider the normal neutrino mass ordering ($m_1<m_2<m_3$) with $m_1=0$, $m_2 = \sqrt{m_{\rm sol}^2}$ and $m_3 = \sqrt{m_{\rm atm}^2}$. In this case, which is equivalent to the one discussed in Ref.~\cite{Granelli:2020ysj}, the matrix $R$ has only one physically relevant angle $z_{23}=x+i\,y$, with real $x,y$. We therefore have 
\begin{equation}\label{eq:R}
R = \begin{pmatrix}
0 & \cos (z_{23})  & \sin (z_{23})  \\
0 & -\sin (z_{23}) & \cos  (z_{23})  \\
1 & 0 & 0 \\
\end{pmatrix} \,.
\end{equation}
In this framework, the mixing parameter between the active light neutrinos and heavy sterile ones takes the following  expression~\cite{Chianese:2018agp}
\begin{eqnarray}
    U^2 & = & \sum_{\alpha\,N} |U_{\alpha (N+3)}|^2 \\
    & = & \frac{m_2-m_3}{2} \frac{\Delta M}{M^2}\cos(2 x) + \frac{(m_2+m_3)}{M} \cosh(2y) \nonumber \,,
    \label{eq:U2}
\end{eqnarray}
where the contribution from $N_3$ is negligible. This is the most relevant quantity that one aims to experimentally constrain. Indeed, there already exist several theoretical and experimental limits, and forecast bounds in the plane $M$-$U^2$ from numerous upcoming, planned and proposed experiments~\cite{Bauer:2019vqk,MATHUSLA:2022sze, Baldini:2021hfw,Feng:2022inv,Abdullahi:2022jlv}. Among the theoretical bounds, the requirement of successful baryogenesis via resonant leptogenesis provides specific allowed regions in the plane $M$-$U^2$, see for instance Ref.~\cite{Klaric:2020phc}.

%================================
\subsection*{Boltzmann equations}
%================================

In order to determine the comoving number density of the baryon asymmetry $\mathcal{N}_B$, we track the evolution of the comoving number densities $\mathcal{N}_{\Delta \ell}$ and $\mathcal{N}_{N_i}$ of the leptonic asymmetry $\Delta \ell$ in the flavour $\ell$ and of $N_i$, respectively. The comoving number densities are simply equal to $\mathcal{N} = n\,a^3$ where $n$ is the physical number density and $a$ the scale factor. In our framework, only $N_1$ and $N_2$ contribute to the final asymmetry since $N_3$ is effectively decoupled. Moreover, we focus on the case where all the RHNs $N_i$ thermalise long before leptogenesis, which we refer to as thermal initial abundance. Under this assumption, the effects of RHNs oscillation ($N_i \leftrightarrow N_j$) has been shown to be subdominant~\cite{Klaric:2021cpi, Akhmedov:1998qx, Drewes:2016gmt}, thus ensuring the validity of the Boltzmann equation formalism.
The Boltzmann equations in terms of \textcolor{red}{$\alpha = \log_{10} a$} read~\cite{Hambye:2016sby,Giudice:2003jh}
\begin{eqnarray} \label{eq:BEN} \frac{{\rm d}\mathcal{N}_{N_i}}{{\rm d}\alpha} &=& \frac{a^3\ln(10)}{H}\left(1-\frac{\mathcal{N}_{N_i}}{\mathcal{N}_N^{\rm eq}}\right)(\gamma_{D} + 2\gamma_{S_s} + 4\gamma_{S_t}) \\
\label{eq:BEL}
\frac{{\rm d}\mathcal{N}_{\Delta \ell}}{{\rm d}\alpha} &=&\frac{a^3\ln(10)}{H} \sum_i \left[ \epsilon_{\ell \ell}^i \left(\frac{\mathcal{N}_{N_i}}{\mathcal{N}_N^{\rm eq}} - 1\right)\gamma_{D} \right. \\
\nonumber &&\left. -P_{\ell\,i}\frac{\mathcal{N}_{\Delta \ell}}{\mathcal{N}_\ell^{\rm eq}} \left(2\gamma_{D} + 2\gamma_{S_t} + \frac{\mathcal{N}_{N_i}}{\mathcal{N}_{N_i}^{\rm eq}} \gamma_{S_s}\right) \right] \,,
\end{eqnarray}
where $H$ is the Hubble rate and $\mathcal{N}_{X}^{\rm eq}$ is the comoving number density of species $X$ in thermal equilibrium with the photon bath. The reaction density $\gamma_{D}$ for the $1\leftrightarrow2$ processes reads as
\begin{eqnarray}
    \gamma_{D} &=&
    \frac{M^3}{\pi^2 z} K_1\left(z\right)\Gamma_{N_i \to \phi L} \Theta(M - M_L + M_\phi) \nonumber \\
    &+& \frac{2 M_H^2 M}{\pi^2 z}K_1\left(z_\phi\right)\Gamma_{\phi \to N_i L} \Theta( M_\phi - M_L + M)
\end{eqnarray}
where $z_\phi = M_\phi / T$, and the quantities $\Gamma_{N_i \to \phi L}$ and $\Gamma_{\phi \to N_i L}$ are the decay widths corrected by the Higgs and lepton thermal masses  The expressions for the rates $\gamma_{S_s}$ and $\gamma_{S_t}$ of the $2 \leftrightarrow 2$ quark and gauge boson scatterings can be found in Ref.~\cite{Giudice:2003jh}.


The Boltzmann equation~\eqref{eq:BEL} for the flavored leptonic asymmetry $\Delta \ell$ depends on the flavoured CP asymmetry parameter $\epsilon^i_{\ell \ell}$ and on the projection probability $P_{\ell i}= |Y_{\ell i}|^2/(Y^\dagger Y)_{ii}$ of heavy neutrino mass state $i$ on to flavour state $\ell$.  the function $\gamma(z)$ describes the temperature dependence of the RHN self-energy cut~\cite{Hambye:2016sby}, which we take from figure~1 in Ref.~\cite{Granelli:2020ysj} without considering the interpolation to account the collinear emissions of soft gauge bosons.

Differently from high-scale leptogenesis where the lepton asymmetry is frozen in long before the sphaleron decoupling at $\Tsphal \approx 132~{\rm GeV}$, in our scenario the lepton asymmetry evolves during and even after the sphaleron decoupling when $M < \Tsphal$. Therefore, to compute the final baryon asymmetry we solve the additional Boltzmann equation accounting for non-instantaneous sphaleron freeze-out~\cite{Eijima:2017cxr}: 

\subsection*{The parameter space of sub-TeV resonant leptogenesis}

We solve the three Boltzmann equations~\eqref{eq:BEN},~\eqref{eq:BEL} and~\eqref{eq:freezeout} assuming $\mathcal{N}_{N_i} = \mathcal{N}^{\rm eq}_{N_i}$ (thermal abundance), $\mathcal{N}_{\Delta \ell} = 0$ and $\mathcal{N}_{B} = 0$ as initial conditions and compute the final baryon asymmetry yield $Y_B = \mathcal{N}_B/\mathcal{S}$ with $\mathcal{S}$ being the comoving entropy density. This has to be compared with the observed value as measured by the Planck experiment~\cite{Planck:2018yye}
\begin{equation}
    Y^{\rm obs}_B = (8.75\pm0.23)\times 10^{-11}\,.
\end{equation}
In the model we consider for sub-TeV resonant leptogenesis, the final yield $Y_B$ depends on four main parameters: the RHN mass scale $M\sim M_1 \sim M_2$, the tiny mass splitting $\Delta M = M_2 - M_1$, and the two angles $x$ and $y$ of the Casas-Ibarra matrix. However, its dependence on $x$ is periodic. In the present analysis, we fix $x=3\pi/4$ which maximises the final baryon asymmetry and, as we will see later, will provide conservative constraints on PBHs whose main effect is the reduction of the asymmetry due to entropy injection (see next section). Hence, we focus on investigating the dependence of $Y_B$ on the remaining three parameters $M$, $\Delta M$ and $y$, which together determine $U^2$ (see  Eq.~\eqref{eq:U2}). This allows us to show the regions achieving successful leptogenesis ($Y_B = \YBobs$) in the plane $M$-$U^2$ for different values of relative mass splitting $\Delta M/M$.
\begin{figure}[t!]
    \centering
    \includegraphics[width = 0.9 \linewidth]{Figures/LeptoPaper2/YBy.pdf}
    \caption{\label{fig:1}  The behaviour of the final baryon asymmetry yield as a function of the angle $y$ for different values of the RHN mass scale $M$ (different line styles) and relative mass splitting $\Delta M /M$ (different colors). The horizontal dotted line represents the observed baryon yield.}
\end{figure}
\begin{figure}[t!]
    \centering
    \includegraphics[width = 0.9 \linewidth]{Figures/LeptoPaper2/YBM.pdf}
    \caption{\label{fig:2} The maximum value of the baryon asymmetry yield (with respect to the angle $y$) as a function of the RHN mass scale $M$, for different relative mass splitting $\Delta M / M$. The horizontal dotted line represents the observed baryon yield.}
\end{figure}

In Fig.~\ref{fig:1} we show the behavior of the baryon asymmetry in some benchmark cases and we compare it with its observed value (horizontal dotted line). In particular, we consider two benchmark values for the RHN mass scale $M=10~{\rm GeV}$ (solid lines) and $M=100~{\rm GeV}$ (dashed lines), for three different values for the relative mass splitting \textcolor{red}{$\Delta M / M = 10^{-12},\,10^{-14},\,10^{-16}$}. In the benchmark cases we show, enough baryon asymmetry can be achieved between an upper and lower limit in $y$. These translate to upper and lower limits in $U^2$, the latter coinciding with the seesaw limit.
\begin{figure}[t!]
    \centering
    \includegraphics[width = 0.9 \linewidth]{Figures/LeptoPaper2/standard.pdf}
    \caption{\label{fig:3} The allowed values for the RHN mass $M$ and the mixing parameter $U^2$ (defined in Eq.~\eqref{eq:U2}) for which the standard sub-TeV resonant leptogenesis is achieved. The different lines correspond to some benchmark values of the relative mass splitting $\Delta M / M$, whose superimposition defines the orange region. The gray area is theoretically excluded by the seesaw mechanism. \textcolor{red}{We report for comparison the projected constraints from the SHiP \cite{SHiP:2018xqw}, SHADOWS \cite{Baldini:2021hfw}, MATHUSLA \cite{MATHUSLA:2022sze} and ANUBIS \cite{Hirsch:2020klk} experiments. }}
\end{figure}

In Fig.~\ref{fig:2} we report the value of $Y_B$ maximised over $y$, as a function of the RHN mass scale, for different mass splittings. Hence, the requirement of successful leptogenesis also defines a lower bound on the RHN mass scale at $\mathcal{O}({\rm GeV})$, which is of high relevance for the experiments devoted to heavy neutral lepton searches.

Hence, we scan over the practically-unobservable relative mass splitting $\Delta M/M$ in the range from \textcolor{red}{$10^{-16}$ to $10^{-11}$}, and we obtain the region in the plane $M$-$U^2$ for which the correct baryon asymmetry is achieved. \textcolor{red}{We choose this range in $\Delta M/M$ in order to maximise the available parameter space for leptogenesis. Considering larger values of the mass splitting does not change our results.} Assuming instead that $N_i$ have a vanishing initial abundance  This is shown in Fig.~\ref{fig:3} by the orange region. The colored lines display different contours in fixed relative mass splitting $\Delta M/M$ for which $Y_B = \YBobs$. The gray area is instead theoretically excluded by the seesaw mechanism. Our results are compatible to the ones presented in Refs.~\cite{Granelli:2020ysj, Klaric:2020phc}. We emphasize that in our treatment we use the full thermally corrected form of the decay rates as done in Ref.~\cite{Hambye:2016sby}, and we improve the calculations of the sphalerons freeze-out by taking into account the non-instantaneous case. Moreover, we underline that we do not interpolate the RHN self-energy function $\gamma$ in Eq.~\eqref{eq:I} in order to approximate the effect of soft gauge scatterings, finding the dip feature in our result for $M < 100~{\rm GeV}$ and high $U^2$ values.




%========================
\section{Results \label{sec:results}}
%========================

We compute the final baryon asymmetry by solving the set of coupled Boltzmann equations including the ones related to the PBH evolution. Hence, we obtain the allowed regions achieving the right final baryon asymmetry in the combined parameter space of RHNs and PBHs, which consists of five parameters: the RHNs mass scale $M$, the RHNs mass splitting $\Delta M$, the real angle $y$ in the Casas-Ibarra matrix, the PBH mass scale $M_{\rm PBH}$, and the PBHs initial abundance $\beta^\prime$.

In Fig.~\ref{fig:4} we show how the RHNs parameter space providing successful leptogenesis is modified due to the presence of PBHs and their evaporation, for different PBHs abundance (left panel) and different PBHs mass (right panel). In the plots, the regions are obtained by superimposing different values for the RHNs mass splitting $\Delta M$ as done in Fig.~\ref{fig:3}. Hence, the effect of PBHs is to shrink the allowed region for the RHNs parameters towards higher masses $M$ and smaller mixing parameters $U^2$. Indeed, the entropy injection from PBHs evaporation reduces the final yield $Y_B$ of baryon asymmetry and tightens the allowed range for the parameters $M$ and $y$ (see Fig.~\ref{fig:1}) in a non-linear way, due to the
non-trivial effects on the sphaleron freeze-out and the
Hubble rate. \textcolor{red}{ We have also reported in Fig.~\ref{fig:4} the projected sensitivity curves for the planned SHiP \cite{SHiP:2018xqw}, SHADOWS \cite{Baldini:2021hfw},MATHUSLA \cite{MATHUSLA:2022sze} and ANUBIS \cite{Hirsch:2020klk} experiments. While these experiments can probe the very edges of resonant leptogenesis parameter space, much larger regions would be ruled out by even the tiny populations of PBHs as illustrated in the figure. Therefore the strong tension between PBHs and leptogenesis can shed light on parameter space well out of reach of direct detection experiments.}

Our findings also have interesting implications on the PBHs parameter space. In Fig.~\ref{fig:5} we report the constraints on the PBHs abundance as a function of the PBHs for different RHNs mass scales. These constraints delineate the regions of PBHs parameter space which are incompatible with sub-TeV resonant leptogenesis at different mass scales M. The smaller the RHNs mass scale, the stronger the constraints on $\beta^\prime$. Indeed, for $M\sim\mathcal{O}({\rm GeV})$ the maximum allowed baryon asymmetry that can be produced by the sub-TeV resonant leptogenesis is of the same order of the one experimentally observed. In the same plot, we show the limits from the observations of Big Bang Nucleosynthesis (shaded gray region) and from the constraints (hatched region) on the energy density of primordial Gravitational Waves~\cite{Papanikolaou:2020qtd,Domenech:2020ssp,Papanikolaou:2022chm}. Moreover, we also report the constrains we placed in our previous study based on the assumption that the baryon asymmetry of the universe is produced through the High-scale Thermal Leptogenesis (HTL)~\cite{Calabrese:2023key}. Hence, the intersection between the regions above the HTL dashed black line and the one above the solid purple line can be regards as the most conservative constraints on the PBHs parameter space placed by the scenarios of baryogenesis via leptogenesis.
\begin{figure}[t!]
    \centering
        \includegraphics[height= 0.9\linewidth]{Figures/LeptoPaper2/constraints.pdf}\,\,
       \caption{\label{fig:5} Upper bounds on the PBHs abundance $\beta^\prime$ defined in Eq.~\eqref{eq:betap} as a function of the PBH mass $M_{\rm PBH}$ for different values of the RHNs mass scale, potentially detectable by upcoming experiments. The hatched region is excluded by the constraints from GW energy density from BBN observations, while the gray one from the PBH evaporation during BBN. For comparison, the dashed line bounds from below the region excluded by the scenario of High-scale Thermal Leptogenesis discussed in Ref.~\cite{Calabrese:2023key}. \textcolor{red}{The gray dotted line bounds from below the region where we observe a period dominated by PBHs in the thermal history of the Universe.}}
\end{figure}


%============================
\section{Conclusions \label{sec:conclusions}}
%============================

In the present paper, we have investigated the impact of PBHs with masses from $10^6$ to $\sim10^9$~g on the predictions of sub-TeV resonant leptogenesis. Differently from the standard scenario of high-scale leptogenesis, in the framework of sub-TeV resonant leptogenesis the observed baryon asymmetry of the Universe is attained through the interactions of (at least) two almost-degenerate Right-Handed Neutrinos with mass from 1~GeV to few TeVs. For this reason, such a scenario is of great interest since it can be probed in laboratories dedicated to the search of heavy neutral leptons through their mixing with active neutrinos.

In the standard cosmological evolution without PBHs, we have solved the Boltzmann equations for the number densities of the Right-Handed Neutrinos and the baryon asymmetry accounting for the non-instantaneous sphaleron freeze-out. In particular, we have assumed the Right-Handed Neutrinos to be initially in thermal equilibrium with the photon bath implying that neutrino oscillations do not play a crucial role in determining the final baryon asymmetry. Hence, we have obtained the standard result (see Fig.~\ref{fig:3}) for the allowed region in the neutrino parameter space which mainly consists of two parameters: the mass scale $M$ of the two Right-Handed Neutrinos and the quantity $U^2$ parameterising the active-sterile neutrino mixing. We have marginalized over the Right-Handed Neutrino mass splitting $\Delta M$.

Then, we have studied the evolution of PBHs whose effects are the modification of the Hubble rate through a matter-domination epoch and the injection of entropy from their evaporation occurring after the sphaleron freeze-out. Interestingly, we have found that the allowed neutrino parameter space shrinks towards higher Right-Handed Neutrino mass scales and smaller active-sterile mixing parameter for different masses and initial abundances of PBHs (see Fig.~\ref{fig:4}). Hence, we have pointed out that the potential laboratory detection of Right-Handed Neutrinos in the mass range from 1 to $\sim 100$~GeV would allowed us to place very competitive constraints on the abundance of PBHs (see Fig.~\ref{fig:5}).


